The Impact of Perceived Tone, Age, and Gender on Voice Assistant Persuasiveness in the Context of Product Recommendations

Voice Assistants (VAs) can assist users in various everyday tasks, but many users are reluctant to rely on VAs for intricate tasks like online shopping. This study aims to examine whether the vocal characteristics of VAs can serve as an effective tool to persuade users and increase user engagement with VAs in online shopping. Prior studies have demonstrated that the perceived tone, age, and gender of a voice influence the perceived persuasiveness of the speaker in interpersonal interactions. Furthermore, persuasion in product communication has been shown to affect purchase decisions in online shopping. We investigate whether variations in a VA voice's perceived tone, age, and gender characteristics can persuade users and ultimately affect their purchase decisions. Our experimental study showed that participants were more persuaded to make purchase decisions by VA voices having positive or neutral tones as well as middle-aged male or younger female voices. Our results suggest that VA designers should offer users the ability to easily customize VA voices with a range of tones, ages, and genders. This customization can enhance user comfort and enjoyment, potentially leading to higher engagement with VAs. Additionally, we discuss the boundaries of ethical persuasion, emphasizing the importance of safeguarding users' interests against unwarranted manipulation.

==> count.tex <==
\usepackage{verbatim}


\newcommand{\quickwordcount}[1]{%
  \immediate\write18{texcount -1 -sum -merge -q #1.tex output.bbl > #1-words.sum }%
  \input{#1-words.sum} words%
}


% Don't count these!
%TC:ignore
\quickwordcount{main}
%TC:endignore
